The Complexity of Non-Monotone Markets

We introduce the notion of non-monotone utilities, which covers a wide variety of utility functions in economic theory. We then prove that it is PPAD-hard to compute an approximate Arrow-Debreu market equilibrium in markets with linear and non-monotone utilities. Building on this result, we settle the long-standing open problem regarding the computation of an approximate Arrow-Debreu market equilibrium in markets with CES utility functions, by proving that it is PPAD-complete when the Constant Elasticity of Substitution parameter \rho is any constant less than -1.

==> Conclusions.tex <==
% !TEX root =  main.tex

\section{Conclusions}

This paper is a first step towards a systematic understanding of what features make the equilibrium analysis of markets computationally hard. We introduced the notion of non-monotone utilities, which covers a wide variety of important utility functions. We then showed that for any family $\calU$ of non-monotone utilities, it is PPAD-hard to compute an approximate equilibrium for a market with utilities that are drawn from $\calU$ or are linear. Using our general approach, and a further, customized analysis, we resolved the long-standing open problem on the complexity of CES markets when the parameter $\rho$ is less than $-1$, showing that for any fixed value of $\rho <-1$, the problem of computing an approximate equilibrium is PPAD-hard.

This work raises clearly many questions. First, can we dispense with the linear functions in the general theorem, i.e., is it true that for any family  $\calU$ of non-monotone utilities, the approximate equilibrium problem is PPAD-hard for markets that use utilities from $\calU$ only? For the important class of CES utilities with (any) $\rho <-1$, we were able to show this, using a deeper analysis of the class of CES utilities, and appropriate~ad\-a\-ptations of the construction. Can a similar approach work in general for all non-monotone utilities?

Second, what other general features of utilities (if any) are there that make the market 
equilibrium~problem hard? Non-monotonicity is connected with markets that can have disconnected sets of
  market equilibria for which currently we do not have any efficient algorithmic methods to deal with. Convexity has been~critical essentially in all tractable cases so far, whether the set
  of market equilibria itself is convex or whether a convex formulation can be obtained after a change of variables. 

Most ambitiously, can we obtain a complexity dichotomy theorem that allows us to classify any family of utility functions (under standard, generally acceptable, mild assumptions for utilities) into those that can be solved efficiently and those that are apparently intractable (PPAD-hard 
  and\hspace{0.026cm}/\hspace{0.026cm}or FIXP-hard)? The present paper takes a first step towards this goal.

\section*{Acknowledgment}

The authors would like to thank Costis Daskalakis and Shang-Hua Teng for very useful
discussions.

==> Proofsketch.tex <==
% !TEX root = main.tex
%\subsection*{PPAD-Hardness of Polymatrix Games}

%Both Theorem \ref{generalhardintro} and the hardness part of Theorem \ref{informalmain} 
%  are proved by giving a polynomial-time reduction from the 
 % following problem called \textbf{\textsc{polymatrix}}.
%The input of the problem is a polymatrix game \cite{Jano} with $n$ players,
% each with two pure strategies.
%Such a game can be described succinctly by a $2n\times 2n$ matrix $\PP$ with entries between $0$ and $1$
%  and $P_{2i-1,2i-1}=P_{2i-1,2i}=P_{2i,2i-1}=P_{2i,2i}$ for all $i\in [n]$.
%We are asked to find a $(1/n)$-well-supported Nash equilibrium, i.e.,
%  a vector $\xx\in \mathbb{R}_+^{2n}$ such that $x_{2i-1}+x_{2i}=1$ and 
%2n ? 2n rational matrix P, with all entries between 0 and 1.
%\begin{align*}
%&\xx^T \cdot \PP_{2i-1} > \xx^T \cdot \PP_{2i} +1/n\ 
%  \hspace{0.03cm}\Rightarrow\hspace{0.03cm}\ x_{2i}=0\\[0.2ex]
%&\xx^T \cdot \PP_{2i} > \xx^T \cdot \PP_{2i-1} +1/n\ \hspace{0.03cm}\Rightarrow\hspace{0.03cm}\ x_{2i-1}=0
%\end{align*}
%for all $i\in [n]$, where we use $\PP_{2i-1}$ and $\PP_{2i}$ to denote the $(2i-1)$th 
%  and $(2i)$th column vectors of $\PP$. 
  
%It was shown in \cite{DGPJournal} (also see \cite{DaskalakisMinmax2}) 
%  that the problem of finding an exact Nash equilibrium of a 
%  two-strategy polymatrix game is PPAD-complete. 
%We show in Section \ref{sec:poly} 
%  that finding a well-supported Nash equilibrium remains PPAD-hard.
%While the hardness of \textbf{\textsc{polymatrix}}
%  only serves in this paper as a bridge to establish Theorem \ref{maintheo:hardness}
%  and \ref{maintheo:general}, we think the result is probably interesting for its own right.
%%\subsection*{Sketch of Hardness Reductions}
%%Indeed we show in Section \ref{CES:reductionsec} that CES markets are (very likely) hard to solve when $\rho<-1$:
%%WGS

\subsection{Proof Sketch of the Hardness Reductions}

We give a rough overview of the constructions for the main results.

For Theorem \ref{maintheo:general},
%\ref{generalhardintro},
  given any $2n\times 2n$ polymatrix game $\PP$ we construct a market
  $M_\PP$ in which the utility of each trader is either linear or from $\calU$.
We then show that given any $\epsilon$-approximate equilibrium $\pp$ of $M_\PP$ 
  for some polynomially small $\epsilon$, we can recover a
  $(1/n)$-well-supported Nash equilibrium in polynomial time.

A building block of our construction is the \emph{linear price-regulating
  markets} \cite{CDDT,VY}.
We let $\tau$ and $\alpha$ denote two positive parameters.
Such a market consists of two traders $T_1,T_2$ and two goods $G_1,G_2$.
$T_i$ owns $\tau$ units of $G_i$, $i\in \{1,2\}$.
The utility of $T_1$ is
  $(1+\alpha)x_1+x_2$ and the utility of $T_2$ is $x_1+(1+\alpha)x_2$.
Let $\pi_i$ denote the price of $G_i$, then we have the 
  following useful property: 
Even if we add more traders to the market, as long as their total
  endowment of $G_1$ and $G_2$ is negligible compared to
  that of $T_1$ and $T_2$, the ratio of
  $\pi_1$ and $\pi_2$ must lie between $(1-\alpha)/(1+\alpha)$ and
  $(1+\alpha)/(1-\alpha)$ at an approximate equilibrium.
 
Our construction starts with the following
  blueprint of encoding   
  a vector $\xx$ of $2\hspace{0.02cm}n$ variables and the $2\hspace{0.02cm}n$ linear forms
  $\xx^T\cdot \PP_j$, $j\in [2n]$, in $M_\PP$. Let $G_1,\ldots,G_{2n}$ and $H_1,\ldots,H_{2n}$
  denote $4\hspace{0.02cm}n$ goods.
Let $\tau$ denote a large enough polynomial in $n$.
Let $\alpha$ and $\beta$ denote two polynomially small parameters with $\alpha\ll \beta$.
For each $i\in [n]$, we first create a price-regulating market
  over $G_{2i-1}$ and $G_{2i}$ with parameters $\tau$ and $\alpha$,
  and a price-regulating market over $H_{2i-1}$ and $H_{2i}$ with parameters
  $\tau$ and $\beta$.
Then for each $i\in [2n]$ and $j\in [2n]$, we add a trader, denoted by $T_{i,j}$, who
  owns $P_{i,j}$ units of $H_{i}$ and is only interested in $G_{j}$.

At this moment, the property of price-regulating markets mentioned above implies that
 at any approximate equilibrium $\pp$, the ratio of $\pi(H_{2i-1})$ and $\pi(H_{2i})$
  is between $(1-\beta)/(1+\beta)$ and $(1+\beta)/(1-\beta)$ 
  and the ratio of $\pi(G_{2i-1})$ and $\pi(G_{2i})$ is between $(1-\alpha)/(1+\alpha)$
  and $(1+\alpha)/(1-\alpha)$, where we use $\pi(G)$ to denote the price of a good $G$ in $\pp$.
Here is some wishful thinking: If for every $i\in [n]$,\vspace{-0.05cm}
$$
\pi(H_{2i-1})+\pi(H_{2i})=\pi(G_{2i-1})+\pi(G_{2i})=2\vspace{0.05cm}
$$
then we can extract a vector $\xx$ from $\pp$ as follows: For each $i\in [2n]$, let
$$
x_{i}=\frac{\pi(H_{i})-(1-\beta)}{2\hspace{0.016cm}\beta}
$$
It is clear that $\xx$ is nonnegative; and $x_{2i-1}+x_{2i}=1$ for all $i\in [n]$.
The linear forms $\xx\cdot \PP_j$ appear in the market $M_\PP$ as follows: The 
  total money that traders $T_{i,j}$, $i\in [2n]$, spend on $G_j$ is\vspace{0.05cm}
$$
\sum_{i\in [2n]} P_{i,j}\cdot \pi(H_i)
= \sum_{i\in [2n]} P_{i,j}\cdot \big(2\hspace{0.02cm}\beta\hspace{0.02cm}x_i+(1-\beta)\big)
=2\hspace{0.02cm}\beta\cdot \xx^T\cdot \PP_j+(1-\beta)\sum_{i\in [2n]} P_{i,j}\vspace{0.05cm}
$$ 
Again with some wishful thinking, we assume that the sums $\sum_{i\in [2n]} P_{i,j}$ 
  are the same for all $j$.
As $\beta\gg \gamma$, $\xx^T\cdot \PP_{2j-1}>\xx^T\cdot \PP_{2j}+1/n$
  would imply that the total demand for $G_{2j-1}$ from traders $T_{i,2j-1}$, $i\in [2n]$ 
  must be strictly larger than that of $G_{2j}$ from traders $T_{i,2j}$, $i\in [2n]$.
To achieve an approximate equilibrium,
  the price-regulating market over $G_{2j-1}$ and $G_{2j}$ 
  must demand strictly more $G_{2j}$ than $G_{2j-1}$, to balance the deficit.
But this can only happen when 
  $\pi(G_{2j-1})$ and $\pi(G_{2j})$ are $1+\alpha$ and $1-\alpha$, respectively.
%giving us $x_{2j-1}=1$ and $x_{2j}=0$ so that the Nash constraint is met.
  
However, what we really need to finish the construction is 
  $\pi(H_{2j-1})=1+\beta$ and $\pi(H_{2j-1})=1-\beta$, so that
$x_{2j-1}=1$, $x_{2j}=0$ and the Nash constraint is met.  
  The big missing piece of the puzzle is then how to enforce
  at any approximate equilibrium the following \emph{ratio amplification}:
$$
\frac{\pi(G_{2j-1})}{\pi(G_{2j})}=\frac{1+\alpha}{1-\alpha}\ \hspace{0.05cm}\Rightarrow\ \hspace{0.03cm}
\frac{\pi(H_{2j-1})}{\pi(H_{2j})}=\frac{1+\beta}{1-\beta}
$$
%as the latter implies $x_{2j-1}=1$ and $x_{2j}=0$, meeting the
%  requirements of a well-supported Nash equilibrium.

It turns out that our goal can be achieved by adding carefully a long chain of copies
  of a non-monotone market $M$ as well as price-regulating markets and traders who transfer money
  between them (like the $T_{i,j}$'s above).
For each $j\in [n]$ we add such a chain that starts from 
  $G_{2j-1},G_{2j}$ and ends at $H_{2j-1},H_{2j}$. 
The~non monotone markets together with price-regulating markets,
  can step-by-step amplify the ratio of two goods,
  either from $(1+\alpha)/(1-\alpha)$ to $(1+\beta)/(1-\beta)$ 
  or from $(1-\alpha)/(1+\alpha)$ to $(1-\beta)/(1+\beta)$.

The tricky part of the construction is that all the actions happen 
  in the local neighborhood of $M$, where the phenomenon of non-monotonicity appears.
Once the chains are added to $M_\PP$, we show 
  that the wishful thinking assumed earlier actually holds, approximately though,
  and we get a polynomial-time reduction.

For Theorem \ref{maintheo:hardness}
%\ref{informalmain}, 
the major challenge is that we can no longer use the
  linear price-regulating markets, but only CES utilities with a fixed $\rho<-1$.
Note that we used the following two properties of price-regulating markets:
  The price ratio is bounded between $(1-\alpha)/(1+\alpha)$ and
  $(1+\alpha)/(1-\alpha)$; and must be equal to one of them if
  the demand of $G_1$ from the price-regulating market is different from
  that of $G_2$.   
The continuous nature of CES utilities however, makes it difficult, if not impossible, to
  construct a CES market that behaves similarly.

Instead we use the simple two-good two-trader market $M$ from \cite{Gjerstad} which is 
  itself a non-monotone market with three isolated market equilibria. 
The high-level picture of the construction is similar to that of Theorem \ref{maintheo:general},
  in which we add to $M_\PP$  
  a long chain of copies of the non-monotone market $M$ for each $j\in [n]$ starting 
  from $G_{2j-1},G_{2j}$ and ending at $H_{2j-1},H_{2j}$.
The proof of correctness, however, is more challenging for which we need
  to first prove a few global properties of $M$.
With these properties we show that whenever the ratio of $\pi(G_{2j-1})$
  and $\pi(G_{2j})$ deviates from $1$ by a non-negligible amount, the chain 
  would amplify the ratio step by step.
By the end of the chain at $H_{2j-1}$ and $H_{2j}$, the ratio converges to one of two constants 
  that correspond to the two nontrivial equilibria of $M$.
Correctness of the reduction then follows.

